Emulating Human Conversations using Convolutional Neural Network-based IR

Conversational agents ("bots") are beginning to be widely used in conversational interfaces. To design a system that is capable of emulating human-like interactions, a conversational layer that can serve as a fabric for chat-like interaction with the agent is needed. In this paper, we introduce a model that employs Information Retrieval by utilizing convolutional deep structured semantic neural network-based features in the ranker to present human-like responses in ongoing conversation with a user. In conversations, accounting for context is critical to the retrieval model; we show that our context-sensitive approach using a Convolutional Deep Structured Semantic Model (cDSSM) with character trigrams significantly outperforms several conventional baselines in terms of the relevance of responses retrieved.

==> 05-results.tex <==
\begin{table}[t]
\begin{tabular}{lll}
\hline
\textbf{Technique}&\textbf{Scores}&\textbf{95\% CI}\\
\hline
IR$_{status}$ & 62.4\% & 3.73 \\
IR$_{status}$+CMM & 63.8\% & 3.78\\
\textbf{DCGM-II + CMM} & 68.4\% & 3.87\\
\hline
SemRel(M,R) + CMM & 79.3\% & 4.15\\
\textbf{SemRel(M,R) + CMM + CCF} & 82\% & 4.23\\
\hline
\end{tabular}
\caption{\small Mean scores assigned by annotators to different systems. The best-performing baseline and experimental systems are shown in bold. {\color{blue}{this table need revamp}}}
\label{mean_scores}
\end{table}

\begin{table}[t]
\begin{tabular}{lll}
\hline
\textbf{Technique}&\textbf{Precision@1}&\textbf{95\% CI}\\
\hline
IR$_{status}$ & 62.4\% & 3.73 \\
IR$_{status}$+CMM & 63.8\% & 3.78\\
\textbf{DCGM-II + CMM} & 68.4\% & 3.87\\
\hline
SemRel(M,R) + CMM & 79.3\% & 4.15\\
\textbf{SemRel(M,R) + CMM + CCF} & 82\% & 4.23\\
\hline
\end{tabular}
\caption{\small Precision of different systems. The best-performing baseline and experimental systems are shown in bold.{\color{blue}{this table need revamp}}}
\label{precision_scores}
\end{table}


\subsection{Quantitative Results}
In Table \ref{precision_scores} we present our results, which clearly shows using deep learnt model to capture deep structured similarity (cDSSM) has given a significant improvement, and outperformed other baselines. Also note that CCF features have played significant role to capture context and do fine tuning of ordering according to context. {\color{blue}{we need to talk about the t-tests etc. here}}

\subsection{Qualitative Analysis}
\label{subsec:qualitative}
Table \ref{qualitative_analysis} shows some examples where our model successfully retrieved a relevant response, and an example where the model retrieved an irrelevant response on our evaluation set as described in Section \ref{ssec:eval}. The $1^{st}$ example (of Relevant result) shows the case where we observe that the response was same with or without considering CCF features, and note that there are no n-gram match in C and R too. It implies that \textit{SemRel(M,R)} was alone sufficient to retrieve a relevant response, because the M itself was quite descriptive and not much dependent on context. It shows that our model has got trained well so as not to overweight contextual features.
However, note in $2^{nd}$ example that \textit{SemSim(C,R)} feature helps get a relevant response as per C. Candidate responses for M \textit{``he is? how so?''}, included \textit{``who he is ?''} and \textit{``aw tell me about it!! he is so hot!''}, which are relevant to M but not so relevant as per C. The $3^{rd}$ example ($1st$ of irrelevant result) shows the case for known limitations of our model. An irrelevant response got retrieved because \textit{``you?''} was the focus of the message and candidates should have been ranked considering ``you?'' as M and ``i am from indonesia.'' as C. Apparently none of the candidates might have got a high score for SemRel(M,R) and CMM feature for M-R lexical match got high importance.

We also show a snippet of actual user chat in Figure \ref{fig:actual_Chat} to fluency and human-like nature of chat from our system. 


